Sim-to-Real Transfer in Deep Reinforcement Learning for Robotics: a Survey

Deep reinforcement learning has recently seen huge success across multiple areas in the robotics domain. Owing to the limitations of gathering real-world data, i.e., sample inefficiency and the cost of collecting it, simulation environments are utilized for training the different agents. This not only aids in providing a potentially infinite data source, but also alleviates safety concerns with real robots. Nonetheless, the gap between the simulated and real worlds degrades the performance of the policies once the models are transferred into real robots. Multiple research efforts are therefore now being directed towards closing this sim-to-real gap and accomplish more efficient policy transfer. Recent years have seen the emergence of multiple methods applicable to different domains, but there is a lack, to the best of our knowledge, of a comprehensive review summarizing and putting into context the different methods. In this survey paper, we cover the fundamental background behind sim-to-real transfer in deep reinforcement learning and overview the main methods being utilized at the moment: domain randomization, domain adaptation, imitation learning, meta-learning and knowledge distillation. We categorize some of the most relevant recent works, and outline the main application scenarios. Finally, we discuss the main opportunities and challenges of the different approaches and point to the most promising directions.

==> sections/old.tex <==
\begin{comment}
\begin{sidewaystable*}
% \begin{table*}
    \centering
    \caption{\footnotesize{Classification of the most relevant publications in Sim2Real Transfer.}}
    \label{tab:papers}
    \footnotesize
    \renewcommand{\arraystretch}{1.42}
    \begin{tabular}{@{}p{0.09\textwidth}p{0.16\textwidth}ccccccccc@{}}
        \toprule
        & \multirow{2}{*}{Description} & Meta & Domain & Continual & Multi-agent & Simulator & Knowledge & Learning & Real & \multirow{2}{*}{Application} \\
        &  & Learning & random. & learning & learning & / Engine & Distillation & Algorithm & Robot/Platform &\\
        \midrule
        %
        %
        %
        \multirow{2}{*}{\textbf{Balaji et al.~\cite{balaji2019deepracer}}} & %
        \scriptsize{DeepRacer: an educational autonomous racing platform with sim2real DRL.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{\shortstack{\cmark\\Distr. rollout}} &        %     <-- Multi-agent learning
        \multirow{2}{*}{\shortstack{Gazebo\\RoboMaker}} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{\shortstack{PPO (Compat. w.\\DQN/DDPG/SAC)}} &        %     <-- Learning algorithm
        \multirow{2}{*}{\shortstack{DeepRacer\\4WD 1:18 Car}} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Autonomous \\ racing}} %     <--  Application
        \\
        %
        %kaspar2020sim2real
        %
        \multirow{2}{*}{\textbf{Traore et al.~\cite{traore2019continual}}} & %
        \scriptsize{Continual RL with policy distillation and sim-to-real transfer.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{\cmark} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{\cmark} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Kaspar et al.~\cite{kaspar2020sim2real}}} & %
        \scriptsize{Sim-to-real transfer for RL without Dynamics Randomization.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Peg-in-Hole \\ manipulation}} %     <--  
        \\
        %
        % 
        %
        \multirow{2}{*}{\textbf{Matas et al.~\cite{matas2018sim}}} & %
        \scriptsize{Sim2Real RL for deformable object manipulation.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Dexterous \\ manipulation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Witman et al.~\cite{witman2019sim}}} & %
        \scriptsize{Sim2Real RL for thermal effects of an atmospheric pressure plasma jet.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Jeong et al.~\cite{jeong2019modelling}}} & %
        \scriptsize{Modelling Generalized Forces with RL for Sim2Real Transfer} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Arndt et al.~\cite{arndt2019meta}}} & %
        \scriptsize{Meta Reinforcement Learning for Sim2Real Domain Adaptation} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Breyer et al.~\cite{breyer2018flexible}}} & %
        \scriptsize{Flexible robotic grasping with Sim2Real RL} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Grasping}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Van Baar et al.~\cite{van2018simulation}}} & %
        \scriptsize{Sim-to-real transfer with robustified policies for robot tasks.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Perturbations ?
        \multirow{2}{*}{\cmark} &        %     <-- Continual learning
        \multirow{2}{*}{\shortstack{\cmark (sim)\\ \xmark (real)}} &        %     <-- Multi-agent learning
        \multirow{2}{*}{\shortstack{MuJoCo\\+Ogre 3D}} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{\cmark} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{\shortstack{A3C (sim)\\Off-policy (real)}} &        %     <-- Learning algorithm
        \multirow{2}{*}{\shortstack{Melfa\\RV-6SL}} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Marble Maze \\ Manipulation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Bassani et al.~\cite{bassani2020learning}}} & %
        \scriptsize{Sim2Real RL for robotic soccer competitions.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Qin et al.~\cite{qin2019sim}}} & %
        \scriptsize{Sim2Real for six-legged robots with DRL and curriculum learning.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Vacaro et al.~\cite{vacaro2019sim}}} & %
        \scriptsize{Sim-to-real in reinforcement learning for everyone} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Low-cost \\ robot arm}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Chaffre et al.~\cite{chaffre2020sim}}} & %
        \scriptsize{Sim-to-Real Transfer with Incremental Environment Complexity} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{\cmark} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{Voxelyze} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{\cmark} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Kaspar et al.~\cite{kasparreinforcement}}} & %
        \scriptsize{Rl with Cartesian Commands and Sim to Real Transfer for Peg in Hole Tasks.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Hundt et al.~\cite{hundt2019good}}} & %
        \scriptsize{Efficient RL for Multi-Step Visual Tasks via Reward Shaping.} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Pedersen et al.~\cite{pedersen2019sim}}} & %
        \scriptsize{Sim-to-Real Transfer for Gripper Pose Estimation with GAN} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robotic \\ Navigation}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Ding et al.~\cite{ding2020sim}}} & %
        \scriptsize{Sim-to-Real Transfer for Optical Tactile Sensing} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{-} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{-} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Tactile \\ sensing}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Muratore et al.~\cite{muratore2020bayesian}}} & %
        \scriptsize{Bayesian Domain Randomization for Sim-to-Real Transfer} & %
        \multirow{2}{*}{-} &        %     <-- Meta learning
        \multirow{2}{*}{\shortstack{\cmark\\(BAYR)}} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{-} &        %     <-- Continual learning
        \multirow{2}{*}{-} &        %     <-- Multi-agent learning
        \multirow{2}{*}{-} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{-} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{\shortstack{RF \\ Classifier}} &        %     <-- Learning algorithm
        \multirow{2}{*}{-} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{swing-up and\\balancing}} %     <--  
        \\
        %
        %
        %
        \multirow{2}{*}{\textbf{Zhao et al.~\cite{wenshuai2020sim2real}}} & %
        \scriptsize{Towards closing the sim-to-real gap in collaborative DRL with perturbances} & %
        \multirow{2}{*}{\xmark} &        %     <-- Meta learning
        \multirow{2}{*}{\shortstack{\cmark\\(custom)}} &        %     <-- Domain randomization / perturbations
        \multirow{2}{*}{\xmark} &        %     <-- Continual learning
        \multirow{2}{*}{\cmark} &        %     <-- Multi-agent learning
        \multirow{2}{*}{Pybullet} &        %     <-- Simulator or physics engine
        \multirow{2}{*}{\xmark} &        %     <-- Knowledge transfer (mult. networks?)
        \multirow{2}{*}{PPO} &        %     <-- Learning algorithm
        \multirow{2}{*}{\shortstack{Kuka\\(sim-only)}} &        %     <-- Real robot / platform
        \multirow{2}{*}{\shortstack{Robot arm\\reacher}} %     <--  
        \\
        \bottomrule
    \end{tabular}
% \end{table*}
\end{sidewaystable*}
\end{comment}
